Composable Energy Policies for Reactive Motion Generation and Reinforcement Learning

Reactive motion generation problems are usually solved by computing actions as a sum of policies. However, these policies are independent of each other and thus, they can have conflicting behaviors when summing their contributions together. We introduce Composable Energy Policies (CEP), a novel framework for modular reactive motion generation. CEP computes the control action by optimization over the product of a set of stochastic policies. This product of policies will provide a high probability to those actions that satisfy all the components and low probability to the others. Optimizing over the product of the policies avoids the detrimental effect of conflicting behaviors between policies choosing an action that satisfies all the objectives. Besides, we show that CEP naturally adapts to the Reinforcement Learning problem allowing us to integrate, in a hierarchical fashion, any distribution as prior, from multimodal distributions to non-smooth distributions and learn a new policy given them.

==> img/models/cep_inference2.tex <==
\tikz{ %

\node[obs] (s0) {$\vs^x$};
\node[latent, right=of s0] (a0) {$\va^x$};

\node[det, above=of s0, xshift=-.95cm](fxz1) {$\vf_{x}^{z_1}$} ;
\node[latent, above=of fxz1, xshift=-.5cm] (sz1) {$\vs^{z_1}$};
\node[latent, above=of fxz1, xshift=.5cm] (az1) {$\va^{z_1}$};
\factoredge {s0,a0} {fxz1} {sz1, az1} ;

\node[det, above=of s0, xshift=.85cm](fxz2) {$\vf_{x}^{z_2}$} ;
\node[latent, above=of fxz2, xshift=-.5cm] (sz2) {$\vs^{z_2}$};
\node[latent, above=of fxz2, xshift=.5cm] (az2) {$\va^{z_2}$};
\factoredge {s0,a0} {fxz2} {sz2, az2} ;

\node[det, above=of a0, xshift=.95cm](fxz3) {$\vf_{x}^{z_3}$} ;
\node[latent, above=of fxz3, xshift=-.5cm] (sz3) {$\vs^{z_3}$};
\node[latent, above=of fxz3, xshift=.5cm] (az3) {$\va^{z_3}$};
\factoredge {s0,a0} {fxz3} {sz3, az3} ;



\factor[above=of sz1, xshift=.5cm] {s0-factor} {} {} {}
\node[obs, above=of s0-factor] (o0) {$o_1$};
\factoredge {sz1,az1} {s0-factor} {o0} ;

\factor[above=of sz2, xshift=.5cm] {s1-factor} {} {} {}
\node[obs, above=of s1-factor] (o1) {$o_2$};
\factoredge {sz2,az2} {s1-factor} {o1} ;

\factor[above=of sz3, xshift=.5cm] {s2-factor} {} {} {}
\node[obs, above=of s2-factor] (o2) {$o_3$};
\factoredge {sz3,az3} {s2-factor} {o2} ;

}

==> img/models/energy_tree_2.tex <==
\tikz{ %
	
	\node[obs] (s0) {$\vs^x$};
	\node[latent, right=of s0, xshift=1.75cm] (a0){$\va^x$};


	\node[det, right=of s0, yshift=0.6cm](fxz1) {$\vf_{x}^{z_1}$} ;
	\node[det, right=of s0, yshift=-0.6cm](fxz2) {$\vf_{x}^{z_2}$} ;

	
	\node[latent, above=of s0] (z1) {$\vs^{z_1}$};
	\node[latent, below=of s0] (z2) {$\vs^{z_2}$};


	\node[latent, above=of a0] (az1) {$\va^{z_1}$};
	\node[latent, below=of a0] (az2) {$\va^{z_2}$};


	\factor[right=of z1, xshift=1.cm] {z1-fac} {$\pi^{z_1}$} {z1} {az1} ; %
	\factor[right=of z2, xshift=1.cm] {z2-fac} {$\pi^{z_2}$} {z2} {az2} ; %
	
	
	\factoredge {s0,a0} {fxz1} {z1, az1} ;
	\factoredge {s0,a0} {fxz2} {z2, az2} ;


	
}

==> img/models/factor_graph.tex <==
\resizebox{0.8\columnwidth}{!}{
    \begin{tikzpicture}
        \Vertex[x=1,y=1]{x1}
        \Vertex[x=2,y=1]{x2}
        \Vertex[x=3,y=1]{x3}
        \Vertex[x=4,y=1]{x4}
        \Vertex[x=5,y=1]{x5}
        \Edge(x1)(x2)
        \Edge(x2)(x3)
        \Edge(x3)(x4)
        \Edge(x4)(x5)
    \end{tikzpicture}
  }

==> tikzlibrarybayesnet.code.tex <==
% tikzlibrary.code.tex
%
% Copyright 2010-2011 by Laura Dietz
% Copyright 2012 by Jaakko Luttinen
%
% The MIT License
%
% See LICENSE file for more details.

% Load other libraries
\usetikzlibrary{shapes}
\usetikzlibrary{fit}
\usetikzlibrary{chains}
\usetikzlibrary{arrows}

% Latent node
\tikzstyle{latent} = [circle,fill=white,draw=black,inner sep=1pt,
minimum size=20pt, font=\fontsize{10}{10}\selectfont, node distance=1]
% Observed node
\tikzstyle{obs} = [latent,fill=gray!25]
% Constant node
\tikzstyle{const} = [rectangle, inner sep=0pt, node distance=1]
% Factor node
\tikzstyle{factor} = [rectangle, fill=black,minimum size=5pt, inner
sep=0pt, node distance=0.4]
% Deterministic node
\tikzstyle{det} = [latent, diamond]

% Plate node
\tikzstyle{plate} = [draw, rectangle, rounded corners, fit=#1]
% Invisible wrapper node
\tikzstyle{wrap} = [inner sep=0pt, fit=#1]
% Gate
\tikzstyle{gate} = [draw, rectangle, dashed, fit=#1]

% Caption node
\tikzstyle{caption} = [font=\footnotesize, node distance=0] %
\tikzstyle{plate caption} = [caption, node distance=0, inner sep=0pt,
below left=5pt and 0pt of #1.south east] %
\tikzstyle{factor caption} = [caption] %
\tikzstyle{every label} += [caption] %

%\pgfdeclarelayer{b}
%\pgfdeclarelayer{f}
%\pgfsetlayers{b,main,f}

% \factoredge [options] {inputs} {factors} {outputs}
\newcommand{\factoredge}[4][]{ %
  % Connect all nodes #2 to all nodes #4 via all factors #3.
  \foreach \f in {#3} { %
    \foreach \x in {#2} { %
      \path (\x) edge[-,#1] (\f) ; %
      %\draw[-,#1] (\x) edge[-] (\f) ; %
    } ;
    \foreach \y in {#4} { %
      \path (\f) edge[->, >={triangle 45}, #1] (\y) ; %
      %\draw[->,#1] (\f) -- (\y) ; %
    } ;
  } ;
}

% \edge [options] {inputs} {outputs}
\newcommand{\edge}[3][]{ %
  % Connect all nodes #2 to all nodes #3.
  \foreach \x in {#2} { %
    \foreach \y in {#3} { %
      \path (\x) edge [->, >={triangle 45}, #1] (\y) ;%
      %\draw[->,#1] (\x) -- (\y) ;%
    } ;
  } ;
}

% \factor [options] {name} {caption} {inputs} {outputs}
\newcommand{\factor}[5][]{ %
  % Draw the factor node. Use alias to allow empty names.
  \node[factor, label={[name=#2-caption]#3}, name=#2, #1,
  alias=#2-alias] {} ; %
  % Connect all inputs to outputs via this factor
  \factoredge {#4} {#2-alias} {#5} ; %
}

% \plate [options] {name} {fitlist} {caption}
\newcommand{\plate}[4][]{ %
  \node[wrap=#3] (#2-wrap) {}; %
  \node[plate caption=#2-wrap] (#2-caption) {#4}; %
  \node[plate=(#2-wrap)(#2-caption), #1] (#2) {}; %
}

% \gate [options] {name} {fitlist} {inputs}
\newcommand{\gate}[4][]{ %
  \node[gate=#3, name=#2, #1, alias=#2-alias] {}; %
  \foreach \x in {#4} { %
    \draw [-*,thick] (\x) -- (#2-alias); %
  } ;%
}

% \vgate {name} {fitlist-left} {caption-left} {fitlist-right}
% {caption-right} {inputs}
\newcommand{\vgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-left) {}; %
  \node[wrap=#4] (#1-right) {}; %
  % Draw the gate
  \node[gate=(#1-left)(#1-right)] (#1) {}; %
  % Add captions
  \node[caption, below left=of #1.north ] (#1-left-caption)
  {#3}; %
  \node[caption, below right=of #1.north ] (#1-right-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.north) -- (#1.south); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}

% \hgate {name} {fitlist-top} {caption-top} {fitlist-bottom}
% {caption-bottom} {inputs}
\newcommand{\hgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-top) {}; %
  \node[wrap=#4] (#1-bottom) {}; %
  % Draw the gate
  \node[gate=(#1-top)(#1-bottom)] (#1) {}; %
  % Add captions
  \node[caption, above right=of #1.west ] (#1-top-caption)
  {#3}; %
  \node[caption, below right=of #1.west ] (#1-bottom-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.west) -- (#1.east); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}

